Language hooks: a modular framework for augmenting LLM reasoning that decouples tool usage from the model and its prompt

Prompting and fine-tuning have emerged as two competing paradigms for augmenting language models with new capabilities, such as the use of tools. Prompting approaches are quick to set up but rely on providing explicit demonstrations of each tool's usage in the model's prompt, thus coupling tool use to the task at hand and limiting generalisation. Fine-tuning removes the need for task-specific demonstrations of tool usage at runtime; however, this ties new capabilities to a single model, thus making already-heavier setup costs a recurring expense. In this paper, we introduce language hooks, a novel framework for augmenting language models with new capabilities that is decoupled both from the model's task-specific prompt and from the model itself. The language hook algorithm interleaves text generation by the base model with the execution of modular programs that trigger conditionally based on the existing text and the available capabilities. Upon triggering, programs may call external tools, auxiliary language models (e.g. using tool specific prompts), and modify the existing context. We benchmark our method against state-of-the-art baselines, find that it outperforms task-aware approaches, and demonstrate its ability to generalise to novel tasks.

==> programs/calculator/correct.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Calculator program: \textbf{Correct} any wrong calculations in the last sentence.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Q1: Rewrite "Text" so as to incorporate the information provided in "Facts". Make a minimal amount of changes and don't add any new information. If the facts are irrelevant you may ignore them and leave the text unchanged.\\
Text:\\
We know that each employee earns 7500 dollars which means that the 10 employee cumulatively earn 45000 dollars.\\
\\
Facts:\\
7500*10 = 75000\\
\\
Fixed text:\\
We know that each employee earns 7500 dollars which means that the 10 employee cumulatively earn 75000 dollars.\\
\\
\\
\\
Q2: Rewrite "Text" so as to incorporate the information provided in "Facts". Make a minimal amount of changes and don't add any new information. If the facts are irrelevant you may ignore them and leave the text unchanged.\\
Text:\\
\{last sentence\}\\
\\
Facts:\\
\{corrected calculation\}\\
\\
Fixed text:\\
\bottomrule
\end{tabular}%
\label{table:program_calculator_correct}
\end{table*}


==> programs/calculator/extract_calculation.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Calculator program: \textbf{Extract} any calculations in the last sentence.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Question: Extract all of the calculations found in the sentence:\\
"That means he spent (13-4) * 9 = 9 * 9 = 81 dollars on ferris wheel tickets."\\
Write down each calculation on a seperate line. If there are no calculations respond with "no calculations". Write calculations in a python parsable format.\\
Answer:\\
(13-4) * 9 = 9 * 9\\
9 * 9 = 81\\
\\
\\
Question: Extract all of the calculations found in the sentence:\\
"Number of Years = $93 / $33852.825\\
\\
Number of Years = 0.0027 years."\\
Write down each calculation on a seperate line. If there are no calculations respond with "no calculations". Write calculations in a python parsable format.\\
Answer:\\
93 / 33852.825 = 0.0027\\
\\
\\
Question: Extract all of the calculations found in the sentence:\\
"Therefore Bob has 3*(5+4)+9*(7+4)=126 toys."\\
Write down each calculation on a seperate line. If there are no calculations respond with "no calculations". Write calculations in a python parsable format.\\
Answer:\\
3*(5+4)+9*(7+4) = 126\\
\\
\\
Question: Extract all of the calculations found in the sentence:\\
"\{last sentence\}"\\
Write down each calculation on a seperate line. If there are no calculations respond with "no calculations". Write calculations in a python parsable format.\\
Answer:\\
\bottomrule
\end{tabular}%
\label{table:program_calculator_extract}
\end{table*}


==> programs/calculator/format_calculation.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Calculator program: \textbf{Format} extracted calculations to run in Python.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Retranscribe the shown calculation as a single-line executable python script. Keep all numbers in the calculation unchanged and do not try and fix the mistakes. Remember to remove dollar signs and other units.\\
\\
\#\#\# Examples\\
\\
Calculation : 13$^\wedge$9 = 117\\
\\
Python script : ```13**9 == 117``` (but calculation is incorrect)\\
\\
Calculation : 13,900dollars×10books = 139,000\\
\\
Python script : ```13900*10 == 139000```\\
\\
\#\#\# Task\\
\\
Calculation : \{extracted calculation\}\\
\\
Python script : \\
\bottomrule
\end{tabular}%
\label{table:program_calculator_format}
\end{table*}


==> programs/retriever/generate_next_sentence.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Retriever program: \textbf{Prompt} the language model to re-generate last sentence}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Answer the question using the references made available to you. Not all references are relevant and you should use as few references as possible. Be careful to only use references:\\
1) Whose relevance is supported by the known information. Their content is already known to be relevant for the final answer.\\
2) Provide new information that will be key towards progressing our answer of the overarching goal.\\
\\
\#\#\# Examples\\
\\
All references (randomly ordered non-comprehensive and sometimes off-topic):\\
{[}1{]} «The Theme | The Theme (Russian: Тема , "Tema " ) is a 1979 Soviet comedy film directed by Gleb Panfilov. It tells the story of an egotistical playwright who thinks of himself as an artist, but who allows the system to make him write conformist plays.»\\
{[}2{]} «The Simpsons Theme | "The Simpsons" Theme", also referred to as "The Simpsons" Main Title Theme" in album releases, is the theme music of the animated television series "The Simpsons". It plays during the opening sequence and was composed by Danny Elfman in 1989, after series creator Matt Groening approached him requesting a retro-style theme. The piece, which took 3 days, 2 hours, 48 minutes, and 19 seconds to create, has been noted by Elfman as the most popular of his career. The theme, as used for the opening sequence, was re-arranged during season 2, and the current arrangement by Alf Clausen was introduced at the beginning of the third season.»\\
{[}3{]} «Theming | Theming refers to "the use of an overarching theme...to create a holistic and integrated spatial organization of a consumer venue." It is also the subject of discourse, discussion, meditation and composition. In an overall sense, theming can be categorized under either "experience"; what an individual sees and feels in their current ‘themed environment’ or "décor"; which is utilized to make an individual remember something through the portrayal of the theme, whether it be generic or specific.»\\
{[}4{]} «The Simpsons | The Simpsons The Simpsons is an American animated sitcom created by Matt Groening for the Fox Broadcasting Company. The series is a satirical depiction of working-class life, epitomized by the Simpson family, which consists of Homer, Marge, Bart, Lisa, and Maggie. The show is set in the fictional town of Springfield and parodies American culture and society, television, and the human condition. The family was conceived by Groening shortly before a solicitation for a series of animated shorts with producer James L. Brooks.»\\
{[}5{]} «Alf Clausen | Alf Clausen Alf Heiberg Clausen (born March 28, 1941) is an American film and television composer. He is best known for his work scoring many episodes of "The Simpsons", of which he had been the sole composer between 1990 and 2017. Clausen has scored or orchestrated music for more than 30 films and television shows, including "Moonlighting", "The Naked Gun", "ALF" and "Ferris Bueller's Day Off". Clausen received an Honorary Doctorate of Music from the prestigious Berklee College of Music in 1996. Clausen was born in Minneapolis, Minnesota and raised in Jamestown, North Dakota. Clausen was interested in music from»\\
\\
Question: """In what year was the creator of the current arrangement of the "Simpson's Theme" born?"""\\
Step-by-step answer: Let's think step by step. From reference {[}1{]} we learn that the creator of the current arrangement of the "Simpson's Theme" is Alf Clausen. From reference {[}5{]} we learn that Alf Clausen was born on March 28, 1941. So the final answer is March 28 1941.\\
Answer{[}March 28 1941{]}\\
\\
---\\
\\
All references (randomly ordered non-comprehensive and sometimes off-topic):\\
{[}1{]} «Training Day | Training Day is a 2001 American neo-noir crime thriller film directed by Antoine Fuqua, and written by David Ayer. Denzel Washington and Ethan Hawke star as two LAPD narcotics officers over a 24-hour period in the gang-ridden neighborhoods of the LAPD Rampart Division and South Central Los Angeles.»\\
{[}2{]} «Old School (film) | Old School is a 2003 American comedy film released by DreamWorks Pictures and The Montecito Picture Company and directed by Todd Phillips. The story was written by Court Crandall, and the film was written by Phillips and Scot Armstrong. The film stars Luke Wilson, Vince Vaughn, and Will Ferrell as three depressed thirty-somethings who seek to re-live their college days by starting a fraternity, and the tribulations they encounter in doing so. Since its release it has gained a massive cult following, since a lot of minor characters in the film went on to have huge careers such as Simon Helberg, Elisha Cuthbert, Rob Corddry and Artie Lange.»\\
{[}3{]} «Training Day (The Office) | "Training Day" is the twentieth episode of the seventh season of the American comedy television series "The Office" and the shows 146th episode overall. It originally aired on NBC on April 14, 2011. The episode was written by Daniel Chun and directed by Paul Lieberstein. This episode marks the first appearance of Deangelo Vickers (Will Ferrell) in the series.»\\
{[}4{]} «Quality Cafe (diner) | The Quality Cafe (also known as Quality Diner) is a now-defunct diner at 1236 West 7th Street in Los Angeles, California. The restaurant ceased to function as a diner in late 2006 but has appeared as a location featured in a number of Hollywood films, including "Training Day", "Old School", "Se7en", "Ghost World", "Gone in 60 Seconds", "The Stepfather", "What's Love Got to Do with It", "Sex and Death 101", and "Catch Me If You Can." It was also featured in Season 1 of the 2007 television series "Mad Men," in the episode "5G".»\\
{[}5{]} «Bad Day for Trains | Bad Day for Trains is the second studio album by Canadian country music singer/songwriter Patricia Conroy, and was released in 1992 by Warner Music Canada. The album was named Album of the Year by the Canadian Country Music Association in 1993.»\\
{[}6{]} «Million Dollar Baby (1941 film) | Million Dollar Baby is a 1941 romantic comedy film directed by Curtis Bernhardt. Released by Warner Bros., the film stars Priscilla Lane, Jeffrey Lynn, and Ronald Reagan, with May Robson and Lee Patrick.»\\
\\
\\
Question: """Who is the director of the 2003 film which has scenes in it filmed at the Quality Cafe in Los Angeles?"""\\
Step-by-step answer: Let's think step by step. From reference {[}4{]} we learn that films which have scenes filmed at the Quality Cafe in Los Angeles include "Training Day", "Old School", "Se7en", "Ghost World", "Gone in 60 Seconds", "The Stepfather", "What's Love Got to Do with It", "Sex and Death 101", and "Catch Me If You Can". From reference {[}2{]} we learn that Old School was released in 2003 and directed by Todd Phillips. So the final answer is Todd Phillips. \\
Answer{[}Todd Phillips{]}\\
\\
\#\#\# Question\\
\\
All references (randomly ordered non-comprehensive and sometimes off-topic):\\
\{references\}\\
\\
Question: """\{question\}"""\\
Step-by-step answer: Let's think step by step.\{rationale with last sentence trimmed\}

\bottomrule
\end{tabular}%
\label{table:program_regenerate_last_sentence}
\end{table*}

==> programs/retriever/generate_search_queries.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Retriever program: \textbf{Generate} search queries}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Your task is to generate a set of 5 searches queries for finding the wikipedia page containing the next relevant facts for progressing our answer. These keywords will be searched against to find the next wikipedia page and so should be:\\
1) comprehensive - they should contain all known knowledge. For example if we are searching for a movie director we should search for `name director` rather than `name`. This is helpful for filtering away similar pages.\\
2) targeted - they should not combine unrelated terms which would be unlikely to be found within a single wikipedia page. Instead they should be specific to one entity on wikipedia. For example they should not combine two unrelated movies.\\
\\
\#\#\# Examples\\
\\
Question: `Are both The New Pornographers and Kings of Leon American rock bands?`\\
Rationale: Let's think step by step. We next need to search on Wikipedia for a page containing the next relevant facts for progressing our answer. Here are 5 variants on a set of keywords against which we could search to find the next wikipedia page:\\
`Kings of Leon`\\
`Kings of Leon band`\\
`New Pornographers`\\
`New Pornographers band`\\
`Kings of Leon country`\\
\\
---\\
\\
Question: `Who is the director of the 2003 film which has scenes in it filmed at the Quality Cafe in Los Angeles?`\\
Rationale: Let's think step by step. Films which have scenes filmed at the Quality Cafe in Los Angeles include Million Dollar Baby, Training Day, and Old School. We next need to search on Wikipedia for a page containing the next relevant facts for progressing our answer. Here are 5 variants on a set of keywords against which we could search to find the next wikipedia page:\\
`Million Dollar Baby`\\
`Million Dollar Baby movie year`\\
`Training day movie`\\
`Old School movie`\\
`Training day movie director`\\
\\
\\
---\\
\\
Question: `In what year was the creator of the current arrangement of the "Simpson's Theme" born?`\\
Rationale: Let's think step by step. The creator of the Simpson's theme is Alf Clausen. We next need to search on Wikipedia for a page containing the next relevant facts for progressing our answer. Here are 5 variants on a set of keywords against which we could search to find the next wikipedia page:\\
`Alf Clausen age`\\
`Al Clausen composer birth year`\\
`Simpson's Alf Clausen born`\\
`Alf Clausen biography`\\
`Alf Clausen`\\
\\
---\\
\\
Question: `The Pineground Bridge formerly carried Depot Road over the Suncook River into a town with a population of what?`\\
Rationale: Let's think step by step. The Pineground Bridge formerly carried Depot Road over the Suncook River into Chichester, New Hampshire. We next need to search on Wikipedia for a page containing the next relevant facts for progressing our answer. Here are 5 variants on a set of keywords against which we could search to find the next wikipedia page:\\
`Chichester New Hampshire town population`\\
`Chichester New Hampshire`\\
`Chichester`\\
`Chichester New Hampshire census`\\
`Chicester census`\\
\\
\#\#\# Task\\
\\
Question: `\{question\}`\\
Rationale: Let's think step by step. \{rationale with last sentence trimmed\} We next need to search on Wikipedia for a page containing the next relevant facts for progressing our answer. Here are 5 variants on a set of keywords against which we could search to find the next wikipedia page: \\
\bottomrule
\end{tabular}%
\label{table:program_generate_search}
\end{table*}


==> prompts/pal_prompts-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\smaller]
\PY{k}{def} \PY{n+nf}{solution}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{Weng earns \PYZdl{}12 an hour for babysitting. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ Yesterday, she just did 50 minutes of babysitting. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ How much did she earn?}\PY{l+s+s2}{\PYZdq{}}
    \PY{n}{hourly\PYZus{}rate} \PY{o}{=} \PY{l+m+mi}{12}   
    \PY{n}{minutes\PYZus{}worked} \PY{o}{=} \PY{l+m+mi}{50}  
    \PY{n}{fraction\PYZus{}of\PYZus{}hour} \PY{o}{=} \PY{n}{minutes\PYZus{}worked} \PY{o}{/} \PY{l+m+mi}{60}  
    \PY{n}{earnings} \PY{o}{=} \PY{n}{hourly\PYZus{}rate} \PY{o}{*} \PY{n}{fraction\PYZus{}of\PYZus{}hour} 
    \PY{n}{result} \PY{o}{=} \PY{n}{earnings}
    \PY{k}{return} \PY{n}{result}


\PY{k}{def} \PY{n+nf}{solution}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{James writes a 3\PYZhy{}page letter to 2 different friends twice a week. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ How many pages does he write a year?}\PY{l+s+s2}{\PYZdq{}}
    \PY{n}{pages\PYZus{}per\PYZus{}letter} \PY{o}{=} \PY{l+m+mi}{3}
    \PY{n}{num\PYZus{}friends} \PY{o}{=} \PY{l+m+mi}{2}
    \PY{n}{letters\PYZus{}per\PYZus{}week} \PY{o}{=} \PY{l+m+mi}{2}
    \PY{n}{weeks\PYZus{}per\PYZus{}year} \PY{o}{=} \PY{l+m+mi}{52}
    \PY{n}{pages\PYZus{}per\PYZus{}year} \PY{o}{=} \PY{n}{pages\PYZus{}per\PYZus{}letter} \PY{o}{*} \PY{n}{num\PYZus{}friends} \PY{o}{*} \PY{n}{letters\PYZus{}per\PYZus{}week} \PY{o}{*} \PY{n}{weeks\PYZus{}per\PYZus{}year}
    \PY{n}{result} \PY{o}{=} \PY{n}{pages\PYZus{}per\PYZus{}year}
    \PY{k}{return} \PY{n}{result}

\PY{k}{def} \PY{n+nf}{solution}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{Mark has a garden with flowers. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ He planted plants of three different colors in it. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ Ten of them are yellow, and there are 80}\PY{l+s+s2}{\PYZpc{}}\PY{l+s+s2}{ more of those in purple. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ There are only 25}\PY{l+s+si}{\PYZpc{} a}\PY{l+s+s2}{s many green flowers as there are yellow and purple flowers. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ How many flowers does Mark have in his garden?}\PY{l+s+s2}{\PYZdq{}}
    \PY{n}{yellow\PYZus{}flowers} \PY{o}{=} \PY{l+m+mi}{10}
    \PY{n}{purple\PYZus{}flowers} \PY{o}{=} \PY{n}{yellow\PYZus{}flowers} \PY{o}{*} \PY{l+m+mf}{1.8}
    \PY{n}{total\PYZus{}flowers} \PY{o}{=} \PY{n}{yellow\PYZus{}flowers} \PY{o}{+} \PY{n}{purple\PYZus{}flowers}
    \PY{n}{green\PYZus{}flowers} \PY{o}{=} \PY{n}{total\PYZus{}flowers} \PY{o}{*} \PY{l+m+mf}{0.25}
    \PY{n}{total\PYZus{}flowers} \PY{o}{+}\PY{o}{=} \PY{n}{green\PYZus{}flowers}
    \PY{n}{result} \PY{o}{=} \PY{n}{total\PYZus{}flowers}
    \PY{k}{return} \PY{n}{result}
\end{Verbatim}


==> prompts/pal_prompts2-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\smaller]
\PY{k}{def} \PY{n+nf}{solution}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{Tina makes \PYZdl{}18.00 an hour. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ If she works more than 8 hours per shift, she is eligible for overtime, }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ which is paid by your hourly wage + 1/2 your hourly wage. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ If she works 10 hours every day for 5 days, how much money does she make?}\PY{l+s+s2}{\PYZdq{}}
    \PY{n}{hourly\PYZus{}wage} \PY{o}{=} \PY{l+m+mf}{18.00}
    \PY{n}{regular\PYZus{}hours} \PY{o}{=} \PY{l+m+mi}{8}
    \PY{n}{overtime\PYZus{}hours} \PY{o}{=} \PY{l+m+mi}{2}
    \PY{n}{overtime\PYZus{}rate} \PY{o}{=} \PY{l+m+mf}{1.5} \PY{o}{*} \PY{n}{hourly\PYZus{}wage}
    \PY{n}{total\PYZus{}hours} \PY{o}{=} \PY{n}{regular\PYZus{}hours} \PY{o}{+} \PY{n}{overtime\PYZus{}hours}
    \PY{n}{total\PYZus{}days} \PY{o}{=} \PY{l+m+mi}{5}
    \PY{n}{total\PYZus{}regular\PYZus{}pay} \PY{o}{=} \PY{n}{hourly\PYZus{}wage} \PY{o}{*} \PY{n}{regular\PYZus{}hours} \PY{o}{*} \PY{n}{total\PYZus{}days}
    \PY{n}{total\PYZus{}overtime\PYZus{}pay} \PY{o}{=} \PY{n}{overtime\PYZus{}rate} \PY{o}{*} \PY{n}{overtime\PYZus{}hours} \PY{o}{*} \PY{n}{total\PYZus{}days}
    \PY{n}{total\PYZus{}pay} \PY{o}{=} \PY{n}{total\PYZus{}regular\PYZus{}pay} \PY{o}{+} \PY{n}{total\PYZus{}overtime\PYZus{}pay}
    \PY{n}{result} \PY{o}{=} \PY{n}{total\PYZus{}pay}
    \PY{k}{return} \PY{n}{result}

\PY{k}{def} \PY{n+nf}{solution}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{A deep\PYZhy{}sea monster rises from the waters once every hundred years to feast }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ on a ship and sate its hunger. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ Over three hundred years, it has consumed 847 people. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ Ships have been built larger over time, so each new ship has twice as }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ many people as the last ship. }\PY{l+s+se}{\PYZbs{}}
\PY{l+s+s2}{        }\PY{l+s+s2}{\PYZbs{}}\PY{l+s+s2}{ How many people were on the ship the monster ate in the first hundred years?}\PY{l+s+s2}{\PYZdq{}}
    \PY{n}{total\PYZus{}people} \PY{o}{=} \PY{l+m+mi}{847}
    \PY{n}{num\PYZus{}ships} \PY{o}{=} \PY{l+m+mi}{3}
    \PY{n}{proportion\PYZus{}on\PYZus{}first\PYZus{}ship} \PY{o}{=} \PY{l+m+mi}{1}
    \PY{n}{proportion\PYZus{}on\PYZus{}second\PYZus{}ship} \PY{o}{=} \PY{n}{proportion\PYZus{}on\PYZus{}first\PYZus{}ship}\PY{o}{*}\PY{l+m+mi}{2}
    \PY{n}{proportion\PYZus{}on\PYZus{}third\PYZus{}ship} \PY{o}{=} \PY{n}{proportion\PYZus{}on\PYZus{}second\PYZus{}ship}\PY{o}{*}\PY{l+m+mi}{2}
    \PY{n}{total\PYZus{}per\PYZus{}proportion} \PY{o}{=} \PY{n}{total\PYZus{}people}\PY{o}{/}\PY{p}{(}\PY{n}{proportion\PYZus{}on\PYZus{}first\PYZus{}ship}\PY{o}{+} \PYZbs{}
        \PY{n}{proportion\PYZus{}on\PYZus{}second\PYZus{}ship}\PY{o}{+}\PY{n}{proportion\PYZus{}on\PYZus{}third\PYZus{}ship}\PY{p}{)}
    \PY{n}{total\PYZus{}on\PYZus{}first\PYZus{}ship} \PY{o}{=} \PY{n}{total\PYZus{}per\PYZus{}proportion}\PY{o}{*} \PY{n}{proportion\PYZus{}on\PYZus{}first\PYZus{}ship}
    \PY{n}{result} \PY{o}{=} \PY{n}{total\PYZus{}on\PYZus{}first\PYZus{}ship}
    \PY{k}{return} \PY{n}{result}
\end{Verbatim}


==> prompts/prompts_2wikimultihop_cot.tex <==
\begin{table*}[tp]
\centering
\caption{base prompt used by CoT and LHs for HotpotQA and 2WikiMultiHopQA.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Answer the following two-hop trivia questions as best you. Always give an answer rather than saying that you don't know. None of the questions are trick questions.\\
Your response should comply to the following template:\\
Question: \$\{\{the question needing answering\}\}\\
Rationale: \$\{\{a step-by-step explanation, where the text is broken down into short sentences, which explicitly shows any facts, guesses and reasoning used to reach your final answer\}\}\\
Answer[\$\{\{your best guess as to the expected answer, obtained using your knowledge and any provided evidence\}\}]\\
\\
---\\
\\
Question: Who is the director of the 2003 film which has scenes in it filmed at the Quality Cafe in Los Angeles?\\
Rationale: Let’s think step by step. Films which have scenes filmed at the Quality Cafe in Los Angeles include Million Dollar Baby, Training Day, and Old School. Among them, Million Dollar Baby was released in 2005. Training Day was released in 2002. Old School was released in 2003. So the correct film is Old School. The director of Old School was Todd Phillips.\\
Answer[Todd Phillips]\\
\\
---\\
\\
Question: Are both The New Pornographers and Kings of Leon American rock bands?\\
Rationale: Let’s think step by step. The New Pornographers are a Canadian indie rock band. Kings of Leon is an American rock band. So one of them is not an American rock band.\\
Answer[no]\\
\\
---\\
\\
Question: In what year was the creator of the current arrangement of the "Simpson's Theme" born?'\\
Rationale: Let’s think step by step. The creator of the current arrangement of the "Simpson's Theme" is Alf Clausen. Alf Clausen was born on March 28, 1941.\\
Answer[1941]\\
\\
---\\
\\
Question: \{question\}\\
Rationale: Let’s think step by step.\\
\bottomrule
\end{tabular}%
\label{table:2wikimultihopqa_cot_prompts}
\end{table*}


==> prompts/prompts_2wikimultihop_react.tex <==
\begin{table*}[tp]
\centering
\caption{ReAct HotpotQA and 2WikiMultihopQA prompts}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
% \textbf{ReAct} \\
Solve a question answering task with interleaving Thought, Action, Observation steps. Thought can reason about the current situation, and Action can be two types:\\
(1) Search{[}text{]}, which searches and returns the first paragraph of Wikipedia articles based on the search term text. If no matches are found, it will return similar entities to search.\\
(2) Finish{[}answer{]}, which returns the answer and finishes the task.\\
\\
Here are some examples.\\
\\
\\
---\\
\\
Question: Who is the director of the 2003 film which has scenes in it filmed at the Quality Cafe in Los Angeles?\\
 Thought 1: I need to search for Quality Cafe and find the director of the 2003 film which has scenes from there.\\
Action 1: Search{[}Quality Cafe{]}\\
Observation 1:\\
{[}1{]} «Quality Cafe | Quality Cafe is the name of two different former locations in Downtown Los Angeles, California.»\\
{[}2{]} «Quality Cafe (diner) | The Quality Cafe (also known as Quality Diner) is a now-defunct diner at 1236 West 7th Street in Los Angeles, California. The restaurant ceased to function as a diner in late 2006 but has appeared as a location featured in a number of Hollywood films, including "Training Day", "Old School", "Se7en", "Ghost World", "Gone in 60 Seconds", "The Stepfather", "What's Love Got to Do with It", "Sex and Death 101", and "Catch Me If You Can." It was also featured in Season 1 of the 2007 television series "Mad Men," in the episode "5G".»\\
{[}3{]} «Quality Cafe (jazz club) | Quality Cafe was a historical restaurant and jazz club located at 1143 East 12th Street near the corner of Central Avenue in Downtown Los Angeles. Quality Four, a jazz quartet founded by saxophonist Paul Howard and featuring young vibraphonist Lionel Hampton, was formed in 1924 to play at Quality Cafe. The band soon became Quality Quintet and then Quality Serenades, and was disbanded after a tour with Hazel Myers later in the same year. On June 7, 1924, the venue changed its name to Humming Bird Cafe and became "one of the hottest nightclubs in the area" under this name.»\\
Thought 2: There are several films filmed at the Quality Cafe (diner). I need to check which one is from 2003.\\
Action 2: Search{[}Training Day{]}\\
Observation 2:\\
{[}1{]} «Training Day | Training Day is a 2001 American neo-noir crime thriller film directed by Antoine Fuqua, and written by David Ayer. Denzel Washington and Ethan Hawke star as two LAPD narcotics officers over a 24-hour period in the gang-ridden neighborhoods of the LAPD Rampart Division and South Central Los Angeles.»\\
{[}2{]} «Training Day (The Office) | "Training Day" is the twentieth episode of the seventh season of the American comedy television series "The Office" and the shows 146th episode overall. It originally aired on NBC on April 14, 2011. The episode was written by Daniel Chun and directed by Paul Lieberstein. This episode marks the first appearance of Deangelo Vickers (Will Ferrell) in the series.»\\
{[}3{]} «Bad Day for Trains | Bad Day for Trains is the second studio album by Canadian country music singer/songwriter Patricia Conroy, and was released in 1992 by Warner Music Canada. The album was named Album of the Year by the Canadian Country Music Association in 1993.»\\
Thought 3: Training Day is from 2001. Let me search instead for Old School.\\
Action 3: Search{[}Old School{]}\\
Oberservation 3:\\
{[}1{]} «Old school | In slang, old school (or old skool) can refer to anything that is from an earlier era or anything that may be considered old-fashioned. The term is commonly used to suggest a high regard for something that has been shown to have lasting value or quality.»\\
{[}2{]} «Old Schools | The Old Schools are part of the University of Cambridge, in the centre of Cambridge, England. The Old Schools house the Cambridge University Offices, which form the main administration for the University.»\\
{[}3{]} «My Old School | "My Old School" is a single drawn from Steely Dan's 1973 album "Countdown to Ecstasy". It reached number 63 on the Billboard charts.»\\
Thought 4: That search didn't return a film. Let me refine my search.\\
Action 4: Search{[}Old School film{]}\\
Observation 4:\\
{[}1{]} «Old School (film) | Old School is a 2003 American comedy film released by DreamWorks Pictures and The Montecito Picture Company and directed by Todd Phillips. The story was written by Court Crandall, and the film was written by Phillips and Scot Armstrong. The film stars Luke Wilson, Vince Vaughn, and Will Ferrell as three depressed thirty-somethings who seek to re-live their college days by starting a fraternity, and the tribulations they encounter in doing so. Since its release it has gained a massive cult following, since a lot of minor characters in the film went on to have huge careers such as Simon Helberg, Elisha Cuthbert, Rob Corddry and Artie Lange.»\\
{[}2{]} «My Old School (film) | My Old School is a 2013 historical documentary created by Jason Allard and Scott Gabrielson.»\\
{[}3{]} «Old School New School (film) | Old School New School is an educational documentary film that examines the nature of creativity. It is produced by Steven Fischer and Diane Leigh Davison.»\\
Thought 5: Old School is a 2003 film. I need to find the director of it. The director of Old School is Todd Phillips.\\
Action 5: Finish{[}Todd Phillips{]}\\
\end{tabular}%
\label{table:2wikimultihop_react_prompts}
\end{table*}


\begin{table*}[tp]
\centering
\begin{tabular}{p{14.5cm}}
\\
---\\
\\
Question: Are both The New Pornographers and Kings of Leon American rock bands?\\
 Thought 1: I need to search for The New Pornographers and Kings of Leon and check if they are both American rock bands.\\
Action 1: Search{[}The New Pornographers{]}\\
Observation 1:\\
{[}1{]} «The New Pornographers | The New Pornographers is a Canadian indie rock band formed in 1997 in Vancouver, British Columbia. Presented as a musical collective of singer-songwriters and musicians from multiple projects, the band has released seven studio albums to critical acclaim for their use of multiple vocalists and elements of power pop incorporated into their music.»\\
{[}2{]} «The Pornographers | The Pornographers is a 1966 Japanese film directed by Shohei Imamura and based on a novel ("Erogotoshitachi") by Akiyuki Nosaka. Its original Japanese title is ""Erogotoshitachi" 
yori Jinruigaku nyūmon" (\japanese{「エロ事師たち」より 人類学入門}), which means 'An introduction to anthropology through the pornographers'. It tells the story of porn film-maker Mr. Subuyan Ogata, whose business is under threat from thieves, the government, and his own family.»\\
{[}3{]} «The Pornographer | The Pornographer (French: Le Pornographe ) is a 2001 French-Canadian drama film written and directed by Bertrand Bonello who co-wrote the music score with Laurie Markovitch. The film features explicit sexual scenes by pornographic actress Ovidie. It won the FIPRESCI Prize (International Critics Week) at the 2001 Cannes Film Festival and was nominated for the Stockholm Film Festival for Bronze Horse.»\\
Thought 2: The New Pornographers are a Canadian indie rock band so I don't need to search for Kings of Leon.\\
Action 2: Finish{[}no{]}\\
\\
---\\
\\
Question: In what year was the creator of the current arrangement of the "Simpson's Theme" born?'\\
 Thought 1: I need to search for Simpson's Theme, find the creator of the current arrangement and then their year of birth.\\
Action 1: Search{[}Simpson's Theme{]}\\
Observation 1:\\
{[}1{]} «The Simpsons Theme | "The Simpsons" Theme", also referred to as "The Simpsons" Main Title Theme" in album releases, is the theme music of the animated television series "The Simpsons". It plays during the opening sequence and was composed by Danny Elfman in 1989, after series creator Matt Groening approached him requesting a retro-style theme. The piece, which took 3 days, 2 hours, 48 minutes, and 19 seconds to create, has been noted by Elfman as the most popular of his career. The theme, as used for the opening sequence, was re-arranged during season 2, and the current arrangement by Alf Clausen was introduced at the beginning of the third season.»\\
{[}2{]} «The Theme | The Theme (Russian: "Tema " ) is a 1979 Soviet comedy film directed by Gleb Panfilov. It tells the story of an egotistical playwright who thinks of himself as an artist, but who allows the system to make him write conformist plays.»\\
{[}3{]} «Theming | Theming refers to "the use of an overarching theme...to create a holistic and integrated spatial organization of a consumer venue." It is also the subject of discourse, discussion, meditation and composition. In an overall sense, theming can be categorized under either "experience"; what an individual sees and feels in their current ‘themed environment’ or "décor"; which is utilized to make an individual remember something through the portrayal of the theme, whether it be generic or specific.»\\
Thought 2: Alf Clausen is the creator of the current arrangement. I need to find his year of birth.\\
Action 2: Search{[}Alf Clausen{]}\\
Observation 2:\\
{[}1{]} «Alf Clausen | Alf Heiberg Clausen (born March 28, 1941) is an American film and television composer. He is best known for his work scoring many episodes of "The Simpsons", of which he had been the sole composer between 1990 and 2017. Clausen has scored or orchestrated music for more than 30 films and television shows, including "Moonlighting", "The Naked Gun", "ALF" and "Ferris Bueller's Day Off".»\\
{[}2{]} «Alf Cock-Clausen | Alf Cock-Clausen (2 March 1886 – 10 July 1983) was a Danish architect. He was active during the transition from Neoclassicism to Functionalism and many of his works show influence from Art Deco. His factory for De Danske Spritfabrikker at Aalborg's harbourfrint was declared a Danish Industrial Heritage Site in 2009. Other works include the headquarters of Guttenberghus (now Egmont Media), now partly converted into the Danish Film Institute, and the Richs Building in Copenhagen.»\\
{[}3{]} «Clausen | Clausen is a Danish patronymic surname, literally meaning "child of Claus", Claus being a German form of the Greek \textNu \textiota \textkappa \textomikron \textlambda \textalpha \textomikron \textvarsigma, Nikolaos, (cf. Nicholas), used in Denmark at least since the 16th century. The spelling variant Klausen has identical pronunciation (as does the often interchangeable Claussen).»\\
Thought 3: Alf Clausen was born in 1941.\\
Action 3: Finish{[}1941{]}\\
\\
---\\
\\
Question: \{question\}\\
\bottomrule
\end{tabular}%
\end{table*}



==> prompts/prompts_GSM8K_cot.tex <==
\begin{table*}[tp]
\centering
% \small
\caption{CoT GSM8K prompts}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Please answer each following question by firstly providing step by step rationale, and then providing the final answer as a single number at the end. Each step should make progress on the rationale little by little patiently, contain reasoning statement involving at most two entities or quantities, and contain at most one mathematical calculation. Each step should not contain calculations that are not explicitly stated, or complex reasoning involving multiple entities or quantities.\\
\\
---\\
\\
Question: Weng earns \$12 an hour for babysitting. Yesterday, she just did 50 minutes of babysitting. How much did she earn?\\
Rationale: Let’s think step by step. Weng earns 12/60=0.2 dollar per minute. Weng worked for 50 minutes, so Weng earned 0.2*50=10 dollars.\\
Numerical final answer: 10\\
\\
---\\
\\
Question: James writes a 3-page letter to 2 different friends twice a week.  How many pages does he write a year?\\
Rationale: Let’s think step by step. James writes each friend 3*2=6 pages a week. So James writes 6*2=12 pages every week. So James writes 12*52=624 pages a year.\\
Numerical final answer: 624\\
\\
---\\
\\
Question: Mark has a garden with flowers. He planted plants of three different colors in it. Ten of them are yellow, and there are 80% more of those in purple. There are only 25% as many green flowers as there are yellow and purple flowers. How many flowers does Mark have in his garden?\\
Rationale: Let’s think step by step. There are 80/100*10=8 more purple flowers than yellow flowers. So there are 10+8=18 purple flowers. Purple and yellow flowers sum up to 10+18=28 flowers. So there are 25/100*28=7 green flowers. So in Mark's garden there are in total 28+7=35 flowers.\\
Numerical final answer: 35\\
\\
---\\
\\
Question: \{question\}\\
Rationale: Let’s think step by step.\\
\bottomrule
\end{tabular}%
\label{table:gsm8k_cot_prompts}
\end{table*}

==> prompts/prompts_GSM8K_pal.tex <==


\lstset{
  language=Python,
  stringstyle=\color{blue},
  breaklines=True,
  literate={\ }{{\ }}1
}

\begin{table*}[tp]
\centering
\small
\caption{PAL GSM8K/GSM8K-Hard prompts}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
    \begin{lstlisting}
    def solution():
        "Weng earns $12 an hour for babysitting. Yesterday, she just
        \ did 50 minutes of babysitting. How much did she earn?"
        hourly_rate = 12
        minutes_worked = 50
        fraction_of_hour = minutes_worked / 60
        earnings = hourly_rate * fraction_of_hour
        result = earnings
        return result
    \end{lstlisting}
    \begin{lstlisting}
    def solution():
        "James writes a 3-page letter to 2 different friends twice a 
        \ week. How many pages does he write a year?"
        pages_per_letter = 3
        num_friends = 2
        letters_per_week = 2
        weeks_per_year = 52
        pages_per_year = pages_per_letter * num_friends * 
            \ letters_per_week * weeks_per_year
        result = pages_per_year
        return result
    \end{lstlisting}
    \begin{lstlisting}
    def solution():
        "Mark has a garden with flowers. He planted plants of three 
        \ different colors in it. Ten of them are yellow, and there 
        \ are 80% more of those in purple. There are only 25% as 
        \ many green flowers as there are yellow and purple flowers. 
        \ How many flowers does Mark have in his garden?"
        yellow_flowers = 10
        purple_flowers = yellow_flowers * 1.8
        total_flowers = yellow_flowers + purple_flowers
        green_flowers = total_flowers * 0.25
        total_flowers += green_flowers
        result = total_flowers
        return result
    \end{lstlisting} \\
    \begin{lstlisting}
    def solution():
        "Tina makes $18.00 an hour. If she works more than 8 hours per shift, she is eligible for overtime, which is paid by your hourly wage + 1/2 your hourly wage. If she works 10 hours every day for 5 days, how much money does she make?"    hourly_wage = 18.00
        regular_hours = 8
        overtime_hours = 2
        overtime_rate = 1.5 * hourly_wage\n    total_hours = regular_hours + overtime_hours
        total_days = 5
        total_regular_pay = hourly_wage * regular_hours * total_days
        total_overtime_pay = overtime_rate * overtime_hours * total_days
        total_pay = total_regular_pay + total_overtime_pay
        result = total_pay
        return result
    \end{lstlisting} \\   
  \end{tabular}
\label{table:gsm8k_pal_prompts}
\end{table*}

\begin{table*}[tp]
\centering
\small
\begin{tabular}{p{14.5cm}}
    \begin{lstlisting}
    def solution():
        "Tina makes $18.00 an hour. If she works more than 8 hours
        \ per shift, she is eligible for overtime, which is paid by
        \ your hourly wage + 1/2 your hourly wage. If she works 10 
        \ hours every day for 5 days, how much money does she make?"
        hourly_wage = 18.00
        regular_hours = 8
        overtime_hours = 2
        overtime_rate = 1.5 * hourly_wage
        total_hours = regular_hours + overtime_hours
        total_days = 5
        total_regular_pay = hourly_wage * regular_hours * total_days
        total_overtime_pay = overtime_rate * overtime_hours * 
            \ total_days
        total_pay = total_regular_pay + total_overtime_pay
        result = total_pay
        return result
    \end{lstlisting}
    
    \begin{lstlisting}
    def solution():
        "A deep-sea monster rises from the waters once every hundred 
        \ years to feast on a ship and sate its hunger. Over three 
        \ hundred years, it has consumed 847 people. Ships have been
        \ built larger over time, so each new ship has twice as many 
        \ people as the last ship. How many people were on the ship 
        \ the monster ate in the first hundred years?"
        total_people = 847
        num_ships = 3
        proportion_on_first_ship = 1
        proportion_on_second_ship = proportion_on_first_ship*2
        proportion_on_third_ship = proportion_on_second_ship*2
        total_per_proportion = total_people/
            \ (proportion_on_first_ship + 
                \ proportion_on_second_ship + 
                    \ proportion_on_third_ship)
        total_on_first_ship = total_per_proportion* 
            \ proportion_on_first_ship
        result = total_on_first_ship
        return result
    \end{lstlisting} \\ 
    
    \bottomrule
  \end{tabular}
\end{table*}

==> prompts/prompts_GSM8K_pal_improved.tex <==
\begin{table*}[tp]
% \centering
% \small
\caption{PAL GSM8K/GSM8K-Hard prompts}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
% \begin{listing}
\input{emnlp2023-latex/prompts/pal_prompts-py}
% \caption{Simple Code to visualize Cartpole Animation}
\label{list:code1}
% \end{listing}
  \end{tabular}
\label{table:gsm8k_pal_prompts}
\end{table*}

\begin{table*}[tp]
% \centering
% \small
% \caption{PAL GSM8K/GSM8K-Hard prompts}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
% \begin{listing}
\input{emnlp2023-latex/prompts/pal_prompts2-py}
% \caption{Simple Code to visualize Cartpole Animation}
\label{list:code1}
% \end{listing}
\bottomrule
  \end{tabular}
\label{table:gsm8k_pal_prompts}
\end{table*}

==> prompts/prompts_GSM8K_react.tex <==

\begin{table*}[tp]
\centering
% \small
\caption{ReAct GSM8K/GSM8K-Hard prompts}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
% \begin{tabular}{ l @{\hspace{32pt}}  l @{\hspace{42pt}}}
% \begin{tabular}{ l @{\hspace{32pt}}  l @{\hspace{42pt}}}
\toprule
% \textbf{ReAct} \\
Solve a question answering task with interleaving Thought, Action, Observation steps. Break down the problem into small substeps. Thought can reason about the current situation, and Action can be two types:\\
(1) Calculator{[}XopY{]}, which at each call calculates a single operation as XopY and returns the answer. Calculator can also solve equations with a single free variable e.g. Calculator{[}3x=6{]}.\\
(2) Finish{[}answer{]}, which returns the answer as an integer and finishes the task.\\
\\
Here are some examples.\\
\\
---\\
\\
Question: Weng earns \$12 an hour for babysitting. Yesterday, she just did 50 minutes of babysitting. How much did she earn?\\
 Thought 1: I need to calculate how much money Weng earns per minute then multiply by the number of minutes Weng worked. Weng earns \$12 an hour and an hour has 60 minutes.\\
Action 1: Calculator{[}12/60{]}\\
Observation 1: 12/60=0.2\\
Thought 2: Weng earns \$0.2 per minute. I now need to calculate how much money Weng earned from working 50 minutes.\\
Action 2: Calculator{[}50*0.2{]}\\
Observation 2: 50*0.2=10\\
Thought 3: Weng earned \$10 in total from working 50 minutes.\\
Action 3: Finish{[}10{]}\\
\\
---\\
\\
Question: James writes a 3-page letter to 2 different friends twice a week.  How many pages does he write a year?\\
 Thought 1: I need to calculate how many pages James writes a week then multiply by the number of weeks in a year.\\
Action 1: Calculator{[}3*2*2{]}\\
Observation 1: 3*2*2=12\\
Thought 2: James writes 12 pages a week. I now need to calculate how many pages we writes in a year. A year has 52 weeks.\\
Action 2: Calculator{[}12*52{]}\\
Observation 2: 12*52=624\\
Thought 3: James writes 624 pages per year.\\
Action 3: Finish{[}624{]}\\
\\
---\\
\\
Question: Mark has a garden with flowers. He planted plants of three different colors in it. Ten of them are yellow, and there are 80% more of those in purple. There are only 25% as many green flowers as there are yellow and purple flowers. How many flowers does Mark have in his garden?\\
 Thought 1: I need to calculate the number of purple flowers. Then I need to calculate the number of green flowers from the number of yellow and purple flowers. Finally I need to add up the number of yellow, purple and green flowers. Mark has 80% more purple flowers than yellow flowers, of which he has 10.\\
Action 1: Calculator{[}1.8*10{]}\\
Observation 1: 1.8*10=18\\
Thought 2: Mark has 18 purple flowers. I now need to calculate how many yellow and purple flowers Mark has.\\
Action 2: Calculator{[}10+18{]}\\
Observation 2: 10+18=28\\
Thought 3: Mark has 28 yellow and purple flowers. I now need to calculate how many green flowers Mark has.\\
Action 3: Calculator{[}0.25*28{]}\\
Observation 3: 0.25*28=7\\
Thought 4: Mark has 7 green flowers. I can now calculate how many flowers Mark has in total by adding up the number of yellow, purple and green flowers.\\
Action 4: Calculator{[}10+18+7{]}\\
Observation 4: 10+18+7=35\\
Thought 5: Mark has 35 flowers in total.\\
Action 5: Finish{[}35{]}\\
\\
---\\
\\
Question: \{question\}\\
\bottomrule
\end{tabular}%
\label{table:gsm8k_prompts}
\end{table*}

==> prompts/prompts_composite_cot.tex <==
\begin{table*}[tp]
\centering
\caption{base prompt used by CoT and LHs for the composite QA dataset.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Answer the following questions as best you. Always give an answer rather than saying that you don't know. None of the questions are trick questions. Use short sentences.\\
Your response should comply to the following template:\\
Question: \$\{\{the question needing answering\}\}\\
Rationale: \$\{\{a step-by-step explanation, where the text is broken down into short sentences, which explicitly shows any facts, guesses and reasoning used to reach your final answer\}\}\\
So the answer to the first part multiplied by the answer to the second part is \$\{\{a number representing your best guess as to the answer\}\}\\
Answer[\$\{\{the answer repeated\}\}]\\
\\
---\\
\\
Question: What is the answer to the first part multiplied by the answer to the second part?\\
First part: The Pineground Bridge formerly carried Depot Road over the Suncook River into a town with a population of what?\\
Second part: James creates a media empire.  He creates a movie for \$2000.  Each DVD of the movie costs \$6 to make.  He sells a DVD for 2.5 times that much.  He sells 500 DVDs a day for 5 days a week.  How much profit does he make in 20 weeks?\\
Rationale: Let’s think step by step. Firstly let's try to answer the first part step by step. The Pineground Bridge formerly carried Depot Road over the Suncook River into Chichester, New Hampshire. Chichester had a population of 2,523 people at the 2010 census. So the answer to the first part is 2523.\\
Then let's try to answer the second part step by step. James sales each DVD for 6*2.5=15 dollars. So James makes a profit of 15-6=9 dollars for each DVD. So each day James makes a profit of 9*500=4500 dollars. So James makes 4500*5=22500 dollars a week. So James makes 22500*20=450000 dollars in 20 weeks. Then after subtracting the cost of creating the movie, James has a profit of 450000-2000=448000 dollars. So the answer to the second part is 448000.\\
So the answer to the first part multiplied by the answer to the second part is 2523*448000=1130304000.\\
Answer[1130304000]\\
\\
---\\
\\
Question: What is the answer to the first part multiplied by the answer to the second part?\\
First part: James writes a 3-page letter to 2 different friends twice a week.  How many pages does he write a year?\\
Second part: Tura Beach, New South Wales is a suburb of a town that had what population at the 2016 census?\\
Rationale: Let’s think step by step. Firstly let's try to answer the first part step by step. James writes each friend 3*2=6 pages a week. So James writes 6*2=12 pages every week. So James writes 12*52=624 pages a year. So the answer to the first part is 624.\\
Then let's try to answer the second part step by step. Tura Beach is suburb of Merimbula, New South Wales, Australia. At the 2016 census, the population of Merimbula was 3,544. So the answer to the second part is 3544.\\
So the answer to the first part multiplied by the answer to the second part is 624*3544=2211456.\\
Answer[2211456]\\
\\
---\\
\\
Question: What is the answer to the first part multiplied by the answer to the second part?\\
First part: In what year did the submarine that sank the Tsushima Maru open to public tours?\\
Second part: Each bird eats 12 beetles per day, each snake eats 3 birds per day, and each jaguar eats 5 snakes per day. If there are 6 jaguars in a forest, how many beetles are eaten each day?\\
Rationale: Let’s think step by step. Firstly let's try to answer the first part step by step. Tsushima Maru was sunk by the submarine USS "Bowfin" during World War II. The submarine USS "Bowfin" has been open to public tours since 1981. So the answer to the first part is 1981.\\
Then let's try to answer the second part step by step. In the forest there are 6 jaguars eating in total 5*6=30 snakes per day. The 30 snakes eat in total 30*3=90 birds per day. The 90 birds eat in total 90*12=1080 beetles per day. So 1080 beetles are eaten in the forest each day. So the answer to the second part is 1080.\\
So the answer to the first part multiplied by the answer to the second part is 1981*1080=2139480.\\
Answer[2139480]\\
\\
---\\
\\
Question: \{question\}\\
Rationale: Let’s think step by step.\\
\bottomrule
\end{tabular}%
\label{table:composite_cot_prompts}
\end{table*}


==> prompts/prompts_composite_react.tex <==
\begin{table*}[tp]
\centering
% \small
\caption{base prompt used by REACT for the composite QA dataset.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Solve a question answering task with interleaving Thought, Action, Observation steps. Thought can reason about the current situation, and Action can be three types:\\
(1) Search[text], which searches and returns the first paragraph of Wikipedia articles based on the search term text. If no matches are found, it will return similar entities to search.\\
(2) Calculator[XopY], which calculates a single operation only as XopY and returns the answer. Calculator can also solve equations with a single free variable e.g. Calculator[3x=6].\\
(3) Finish[answer], which returns the answer and finishes the task.\\
\\
Here are some examples.\\
\\
\\
---\\
\\
Question: What is the answer to the first part multiplied by the answer to the second part?\\
First part: The Pineground Bridge formerly carried Depot Road over the Suncook River into a town with a population of what?\\
Second part: James creates a media empire.  He creates a movie for \$2000.  Each DVD of the movie costs \$6 to make.  He sells a DVD for 2.5 times that much.  He sells 500 DVDs a day for 5 days a week.  How much profit does he make in 20 weeks?\\
 Thought 1: I need to search for The Pineground Bridge.\\
Action 1: Search[The Pineground Bridge]\\
Observation 1:\\
{[}1{]} «Pineground Bridge | The Pineground Bridge, also known as the Depot Road Bridge or the Thunder Bridge, is a through-type lenticular truss bridge that formerly carried Depot Road over the Suncook River in Chichester, New Hampshire. The bridge was built in 1887 by the Berlin Iron Bridge Co., and is the only one of its type (and only one of for lenticular truss bridges of any type, as of 2004) in the state. It is 96 ft long and 16 ft wide, and rises 15 ft above the river. It is mounted on abutments made of unmortarted ashlar granite. The decking and rails are made of wood. The bridge has not undergone major alterations since its construction. Some of its stringers were replaced during the 1981-2 restoration, wooden parts were also replaced, and a number of decorative parts have been lost over the years.»\\
{[}2{]} «New Bridge (Dublin) | The New Bridge is a bridge over the River Dodder in Dublin. The bridge is also known as Herbert's Bridge or Lansdowne Bridge. The bridge is part of Lansdowne Road.»\\
{[}3{]} «Bridge therapy | Bridge therapy is therapy intended, in transportation metaphor, to serve as a figurative bridge to another stage of therapy or health, carrying a patient past a challenging period of some kind. There are various types of bridge therapy, such as bridge to transplant, bridge to candidacy, bridge to decision, bridge to recovery, and anticoagulation bridge (such as heparin bridge). Bridge therapy exists in contrast to destination therapy, which is the figurative destination rather than a bridge to something else.»\\
Thought 2: The Pineground Bridge formerly carried Depot Road over the Suncook River in Chichester, New Hampshire. I now need to search for Chichester, New Hampshire.\\
Action 2: Search[Chichester, New Hampshire]\\
Observation 2:\\
{[}1{]} «Chichester, New Hampshire | Chichester is a town in Merrimack County, New Hampshire, United States. The population was 2,523 at the 2010 census.»\\
{[}2{]} «Robert Trigges | Robert Trigges (by 1508-1550/1551), of St. Peter's, Chichester, Sussex and Chawton, Hampshire, was an English politician.»\\
{[}3{]} «Gabrielle Brune | Gabrielle Brune (12 February 1912 in Bournemouth, Hampshire – 18 January 2005 in Chichester, Sussex) was a British actress.»\\
Thought 3: Chichester has a population of 2,523 so the answer to the first part is 2523. I now need to solve the second part. I will work out the revenue per single DVD sale.\\
Action 3: Calculator[6*2.5]\\
Observation 3: 6*2.5=15\\
Thought 4: I will now work out the profit per DVD.\\
Action 4: Calculator[15-6]\\
Observation 4: 15-6=9\\
Thought 5: So James makes \$9 profit per DVD. I will now calculate his daily profit.\\
Action 5: Calculator[9*500]\\
Observation 5: 9*500=4500\\
Thought 6: James makes \$4500 profit a day. I can now calculate his total profit from DVD sales.\\
Action 6: Calculator[4500*5*20]\\
Observation 6: 4500*5*20=450000\\
Thought 7: James makes \$450000 in total. I now need to subtract the cost of movie creation to get his final profit.\\
Action 7: Calculator[450000-2000]\\
Observation 7: 450000-2000=448000\\
Thought 8: So James makes 448000 as his final profit in 20 weeks. So the answer to the second part is 448000. I can now calculate the answer to the first part multiplied by the answer to the second part.\\
Action 8: Calculator[2523*448000]\\
Observation 8: 2523*448000=1130304000\\
Thought 9: So the answer to the first part multiplied by the answer to the second part is 1130304000.\\
Action 9: Finish[1130304000]\\
\\
---\\
\\
Question: What is the answer to the first part multiplied by the answer to the second part?\\
First part: James writes a 3-page letter to 2 different friends twice a week.  How many pages does he write a year?\\
Second part: Tura Beach, New South Wales is a suburb of a town that had what population at the 2016 census?\\
 Thought 1: I need to search for The Pineground Bridge.\\
Action 1: Search[The Pineground Bridge]\\
Observation 1:\\
{[}1{]} «Pineground Bridge | The Pineground Bridge, also known as the Depot Road Bridge or the Thunder Bridge, is a through-type lenticular truss bridge that formerly carried Depot Road over the Suncook River in Chichester, New Hampshire. The bridge was built in 1887 by the Berlin Iron Bridge Co., and is the only one of its type (and only one of for lenticular truss bridges of any type, as of 2004) in the state. It is 96 ft long and 16 ft wide, and rises 15 ft above the river. It is mounted on abutments made of unmortarted ashlar granite. The decking and rails are made of wood. The bridge has not undergone major alterations since its construction. Some of its stringers were replaced during the 1981-2 restoration, wooden parts were also replaced, and a number of decorative parts have been lost over the years.»\\
{[}2{]} «New Bridge (Dublin) | The New Bridge is a bridge over the River Dodder in Dublin. The bridge is also known as Herbert's Bridge or Lansdowne Bridge. The bridge is part of Lansdowne Road.»\\
{[}3{]} «Bridge therapy | Bridge therapy is therapy intended, in transportation metaphor, to serve as a figurative bridge to another stage of therapy or health, carrying a patient past a challenging period of some kind. There are various types of bridge therapy, such as bridge to transplant, bridge to candidacy, bridge to decision, bridge to recovery, and anticoagulation bridge (such as heparin bridge). Bridge therapy exists in contrast to destination therapy, which is the figurative destination rather than a bridge to something else.»\\
Thought 2: The Pineground Bridge formerly carried Depot Road over the Suncook River in Chichester, New Hampshire. I now need to search for Chichester, New Hampshire.\\
Action 2: Search[Chichester, New Hampshire]\\
Observation 2:\\
{[}1{]} «Chichester, New Hampshire | Chichester is a town in Merrimack County, New Hampshire, United States. The population was 2,523 at the 2010 census.»\\
{[}2{]} «Robert Trigges | Robert Trigges (by 1508-1550/1551), of St. Peter's, Chichester, Sussex and Chawton, Hampshire, was an English politician.»\\
{[}3{]} «Gabrielle Brune | Gabrielle Brune (12 February 1912 in Bournemouth, Hampshire – 18 January 2005 in Chichester, Sussex) was a British actress.»\\
Thought 3: Chichester has a population of 2,523 so the answer to the first part is 2523. I now need to solve the second part. I will work out the revenue per single DVD sale.\\
Action 3: Calculator[6*2.5]\\
Observation 3: 6*2.5=15\\
Thought 4: I will now work out the profit per DVD.\\
Action 4: Calculator[15-6]\\
Observation 4: 15-6=9\\
Thought 5: So James makes \$9 profit per DVD. I will now calculate his daily profit.\\
Action 5: Calculator[9*500]\\
Observation 5: 9*500=4500\\
Thought 6: James makes \$4500 profit a day. I can now calculate his total profit from DVD sales.\\
Action 6: Calculator[4500*5*20]\\
Observation 6: 4500*5*20=450000\\
Thought 7: James makes \$450000 in total. I now need to subtract the cost of movie creation to get his final profit.\\
Action 7: Calculator[450000-2000]\\
Observation 7: 450000-2000=448000\\
Thought 8: So James makes 448000 as his final profit in 20 weeks. So the answer to the second part is 448000. I can now calculate the answer to the first part multiplied by the answer to the second part.\\
Action 8: Calculator[2523*448000]\\
Observation 8: 2523*448000=1130304000\\
Thought 9: So the answer to the first part multiplied by the answer to the second part is 1130304000.\\
Action 9: Finish[1130304000]\\
\\
---\\
\\
Question: \{question\}\\
\bottomrule
\end{tabular}%
\label{table:composite_react_prompts}
\end{table*}


==> table_cost.tex <==
\begin{table*}[tp]
\centering
\small
\caption{LLM usage and costs}
\vspace{2mm}
\begin{tabular}{ l @{\hspace{32pt}} cc @{\hspace{42pt}}  cc @{\hspace{42pt}} cc @{\hspace{8pt}}}
\toprule
& \multicolumn{2}{c@{\hspace{42pt}}}{\textbf{GSM8k}}
& \multicolumn{2}{c@{\hspace{42pt}}}{\textbf{GSM8kHard}}\\
\midrule
\textbf{ReAct} with calculator tools  & -- & -- & -- & -- \\
\textbf{CoT} & -- & -- &  -- & --  \\
\textbf{PAL on gpt-turbo-3.5} & -- & -- &  -- & --  \\
\midrule
\textbf{Language hooks} & -- & -- & \textbf{--} & \textbf{--} \\
\bottomrule
\end{tabular}%
\label{table:cost}
\end{table*}

==> trigger_ablation_barplot.tex <==
\begin{figure*}[t]
  \centering
\includegraphics[width=\textwidth]{emnlp2023-latex/varying_trigger_rate_barplot_ablation.png}
§  \caption{F1 scores for varying trigger rates. CoT and Base trigger rate F1 scores correspond to the results shown in Section ???\ref{experiments}.}
  \label{fig:schematic}
\end{figure*}




==> triggers/calculator.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Calculator trigger prompt (evaluated on \texttt{curie}). Log-probabilities are evaluated only on the green text.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Classify each sentence as containing or not containing mathematical calculations.\\
The sentence "Firstly let's try to answer the first question step by step." contains no mathematics\\
The sentence "Bob already had 5 books and buys 10 books which means he now owns 10+5 = 15 books." contains mathematics\\
The sentence "According to reference [1] the population of the USA in 2005 was 2000000." contains no mathematics\\
The sentence "Mario's original salary was 4000/1.4=2857.14 dollars" contains mathematics\\
The sentence "So she needs to copy 20*2=40 pages before the end of the day." contains mathematics\\
The sentence "The answer to the first question is 2005." contains no mathematics\\
The sentence "The second world war started on the 18 of March 1939." contains no mathematics\\
The sentence "\{last sentence\}" contains\colorbox{lime}{ mathematics} \\
\bottomrule
\end{tabular}%
\label{table:trigger_calculator}
\end{table*}


==> triggers/guardrail.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Guardrail trigger prompt (evaluated on \texttt{curie}). Log-probabilities are evaluated only on the green text.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Identify the sentences where information was failed to be found.\\
The sentence 'So Legend Of The Sea Wolf came out first.' did not fail to find information\\
The sentence 'There is no movie called Education Of A Prince.' failed to find information\\
The sentence 'We need to find the birth years of the directors of both films.' did not fail to find information\\
The sentence 'I couldn't find any information on Edward Bibring's wife or her occupation.' failed to find information\\
The sentence 'Joe Jackson was nominated for a Grammy Award in 1979 for Best Male Pop Vocal Performance.' did no fail to find information\\
The sentence 'Without any additional information, we cannot determine the birth order of Alexey Volkonsky and Wanderley Oliveira.' failed to find information\\
The sentence 'Answer[Life Is Hot In Cracktown]' did not fail to find information\\
The sentence '\{last sentence\}'\colorbox{lime}{ failed to find}\\
\bottomrule
\end{tabular}%
\label{table:trigger_guardrail}
\end{table*}

==> triggers/retriever.tex <==
\begin{table*}[tp]
\centering
\small
\caption{Retriever trigger prompt (evaluated on \texttt{curie}). Log-probabilities are evaluated only on the green text.}
\vspace{2mm}
\begin{tabular}{p{14.5cm}}
\toprule
Question: \{question\}\\
Answer:\\
Let's think step by step. \{rational\} In order to write down the sentence "\{last sentence\}" I had to\colorbox{lime}{ research facts}\\
\bottomrule
\end{tabular}%
\label{table:trigger_retriever}
\end{table*}
